A Context-Aware Computational Approach for Measuring Vocal Entrainment in Dyadic Conversations

Vocal entrainment is a social adaptation mechanism in human interaction, knowledge of which can offer useful insights to an individual's cognitive-behavioral characteristics. We propose a context-aware approach for measuring vocal entrainment in dyadic conversations. We use conformers(a combination of convolutional network and transformer) for capturing both short-term and long-term conversational context to model entrainment patterns in interactions across different domains. Specifically we use cross-subject attention layers to learn intra- as well as inter-personal signals from dyadic conversations. We first validate the proposed method based on classification experiments to distinguish between real(consistent) and fake(inconsistent/shuffled) conversations. Experimental results on interactions involving individuals with Autism Spectrum Disorder also show evidence of a statistically-significant association between the introduced entrainment measure and clinical scores relevant to symptoms, including across gender and age groups.

==> experiment.tex <==
\label{sec:ex}

\begin{itemize}
    \item ML-SSP: multi-lingual self-supervised pretraining
    \item LA-ML-SSP: language-adapted ML-SSP
    \item Opt. LAL: optimum language-adapted learning with LEAP
\end{itemize}

\begin{table*}[h]
   \begin{minipage}{\textwidth}
	\centering
	\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|}
	    \hline
	           & de & it & ru & fr & fr-CA & es & es-MX & pt & pt-BR & AVG. \\ \hline\hline
        Baseline  &  &  & &  & & & & & & \\ \hline
        ML-SSP    &  &  & &  & & & & & & \\ \hline
        LA-ML-SSP &  &  & &  & & & & & & \\ \hline
        Opt. LAL  &  &  & &  & & & & & & \\ \hline
	\end{tabular}
	\caption{WER with the single multi-lingual network on the in-domain language data.}
    \label{tab:ml-indomain}
    \end{minipage}
    %\vspace{-0.3cm}
    \hfill
    \begin{minipage}{\textwidth}
    \centering
	\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|}
	    \hline
	           & de & it & ru & fr & fr-CA & es & es-MX & pt & pt-BR & AVG. \\ \hline\hline
        Baseline  &  &  & &  & & & & & & \\ \hline
        ML-SSP    &  &  & &  & & & & & & \\ \hline
        LA-ML-SSP &  &  & &  & & & & & & \\ \hline
        Opt. LAL &  &  & &  & & & & & & \\ \hline
	\end{tabular}
	\caption{WER with the fine-tuned language-dependent network on the in-domain language data.}
    \label{tab:ft-indomain}
    \end{minipage}
\end{table*}\hfill

Table~\ref{tab:ml-indomain} shows the word error rate (WER) with each single multi-lingual network on the in-domain language data. 
\newpage

\begin{table}[b]
	\centering
	\begin{tabular}{|c||c|c|c|}
	    \hline
	              & \multicolumn{3}{|c|}{ro} \\ \hline\hline
                  & 50 hrs. & 100 hrs. & 690 hrs.   \\ \hline
        Baseline  &  & &  \\ \hline
        ML-SSP &  & &  \\ \hline
        Opt. LAL &  & &  \\ \hline
	\end{tabular}
	\caption{WER on the new language data.}
    \label{tab:outdomain}
    %\vspace{-0.3cm}
\end{table}

